Multi Resolution Analysis (MRA) for Approximate Self-Attention

Transformers have emerged as a preferred model for many tasks in natural langugage processing and vision. Recent efforts on training and deploying Transformers more efficiently have identified many strategies to approximate the self-attention matrix, a key module in a Transformer architecture. Effective ideas include various prespecified sparsity patterns, low-rank basis expansions and combinations thereof. In this paper, we revisit classical Multiresolution Analysis (MRA) concepts such as Wavelets, whose potential value in this setting remains underexplored thus far. We show that simple approximations based on empirical feedback and design choices informed by modern hardware and implementation challenges, eventually yield a MRA-based approach for self-attention with an excellent performance profile across most criteria of interest. We undertake an extensive set of experiments and demonstrate that this multi-resolution scheme outperforms most efficient self-attention proposals and is favorable for both short and long sequences. Code is available at \url{https://github.com/mlpen/mra-attention}.

==> inserts/bslr_demo_figure.tex <==


\begin{figure*}[!htbp]
\centering
\includegraphics[width=6.2in]{figs/bslr_demo.pdf}
\caption{Illustration of Approximation Algorithm}
\label{fig:bslr_demo}
\end{figure*}

==> inserts/multi_res.tex <==

% \begin{wrapfigure}[12]{l}{0.25\textwidth}
\begin{figure}[!htbp]
\centering
\includegraphics[width=0.8in]{figs/multires.pdf}
\caption{An example of 3-resolution approximation of $8 \times 8$ matrix. Entries within the same square blocks has the same values. }
\label{fig:multi_res}
\end{figure}
% \end{wrapfigure}

==> inserts/roberta_512_table.tex <==


\begin{table*}[!htbp]
\begin{center}
\begin{scriptsize}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l|cccccc|ccccc}
\toprule
Method & Time & Mem & \multicolumn{2}{c}{MLM} & \multicolumn{2}{c}{MNLI}  \\
 & \tiny{ms} & \tiny{MB} & \tiny{Before} & \tiny{After} & \tiny{m} & \tiny{mm} \\
\midrule
Transformer  &  {\transparent{0.8}{0.86}}  &  {\transparent{0.3}{71.0}}  &  {\textbf{73.1}}  &  {\textbf{74.0}}  &  {\textbf{87.4}}  &  {\textbf{87.3}}  &  {\transparent{0.8}{0.41}}  &  {\transparent{0.3}{35.5}}  &  {\textbf{57.0}}  &  {\transparent{0.8}{73.1}}  &  {\transparent{0.8}{73.9}} \\
Performer  &  {\transparent{0.3}{1.29}}  &  {\transparent{0.3}{62.8}}  &  {\transparent{0.8}{6.8}}  &  {\transparent{0.3}{63.1}}  &  {\transparent{0.3}{32.7}}  &  {\transparent{0.3}{33.0}}  &  {\transparent{0.3}{0.63}}  &  {\transparent{0.3}{31.4}}  &  {\transparent{0.3}{48.6}}  &  {\transparent{0.3}{70.1}}  &  {\transparent{0.3}{70.5}} \\
Linformer  &  {\textbf{0.74}}  &  {\transparent{0.8}{54.5}}  &  {\transparent{0.3}{1.0}}  &  {\transparent{0.3}{5.6}}  &  {\transparent{0.8}{35.4}}  &  {\transparent{0.8}{35.2}}  &  {\textbf{0.35}}  &  {\transparent{0.8}{27.2}}  &  {\transparent{0.8}{53.5}}  &  {\transparent{0.8}{73.1}}  &  {\transparent{0.8}{73.5}} \\
SOFT  &  {\textbf{0.86}}  &  {\textbf{34.0}}  &  {\transparent{0.8}{10.9}}  &  {\transparent{0.3}{25.0}}  &  {\transparent{0.3}{32.7}}  &  {\transparent{0.3}{33.0}}  &  {\transparent{0.8}{0.43}}  &  {\textbf{17.0}}  &  {\transparent{0.3}{42.8}}  &  {\transparent{0.3}{64.6}}  &  {\transparent{0.3}{65.6}} \\
SOFT + Conv  &  {\transparent{0.8}{1.02}}  &  {\transparent{0.8}{35.5}}  &  {\transparent{0.3}{1.0}}  &  {\transparent{0.8}{65.5}}  &  {\transparent{0.8}{74.9}}  &  {\transparent{0.8}{75.0}}  &  {\transparent{0.8}{0.53}}  &  {\transparent{0.8}{17.8}}  &  {\transparent{0.8}{56.7}}  &  {\transparent{0.3}{71.1}}  &  {\transparent{0.3}{71.9}} \\
Nystromformer  &  {\textbf{0.71}}  &  {\transparent{0.8}{34.8}}  &  {\transparent{0.8}{17.2}}  &  {\transparent{0.8}{68.2}}  &  {\transparent{0.8}{35.4}}  &  {\transparent{0.8}{35.2}}  &  {\textbf{0.34}}  &  {\transparent{0.8}{17.4}}  &  {\transparent{0.3}{53.1}}  &  {\transparent{0.3}{71.0}}  &  {\transparent{0.3}{71.8}} \\
Nystrom + Conv  &  {\transparent{0.8}{0.88}}  &  {\transparent{0.8}{37.2}}  &  {\transparent{0.3}{1.4}}  &  {\transparent{0.8}{70.9}}  &  {\transparent{0.8}{85.1}}  &  {\transparent{0.8}{84.6}}  &  {\transparent{0.8}{0.45}}  &  {\transparent{0.8}{18.6}}  &  {\textbf{57.3}}  &  {\transparent{0.8}{73.3}}  &  {\transparent{0.8}{73.9}} \\
Reformer  &  {\transparent{0.3}{ - }}  &  {\transparent{0.3}{ - }}  &  {\transparent{0.3}{ - }}  &  {\transparent{0.3}{ - }}  &  {\transparent{0.3}{ - }}  &  {\transparent{0.3}{ - }}  &  {\textbf{0.39}}  &  {\textbf{16.4}}  &  {\transparent{0.3}{52.4}}  &  {\textbf{74.0}}  &  {\textbf{74.6}} \\
Reformer  &  {\transparent{0.8}{1.23}}  &  {\transparent{0.8}{59.4}}  &  {\transparent{0.3}{0.7}}  &  {\transparent{0.8}{69.5}}  &  {\transparent{0.8}{84.9}}  &  {\transparent{0.8}{85.0}}  &  {\transparent{0.3}{0.61}}  &  {\transparent{0.3}{29.6}}  &  {\transparent{0.8}{55.6}}  &  {\textbf{75.0}}  &  {\textbf{75.8}} \\
Longformer  &  {\transparent{0.3}{1.30}}  &  {\transparent{0.8}{43.3}}  &  {\transparent{0.8}{66.0}}  &  {\transparent{0.8}{71.2}}  &  {\transparent{0.8}{85.6}}  &  {\transparent{0.8}{85.4}}  &  {\transparent{0.3}{0.61}}  &  {\transparent{0.8}{21.6}}  &  {\transparent{0.8}{54.7}}  &  {\transparent{0.8}{72.2}}  &  {\transparent{0.8}{73.6}} \\
Longformer  &  {\transparent{0.3}{2.31}}  &  {\transparent{0.3}{62.5}}  &  {\textbf{71.9}}  &  {\textbf{73.2}}  &  {\textbf{87.0}}  &  {\textbf{87.1}}  &  {\transparent{0.3}{1.10}}  &  {\transparent{0.3}{31.4}}  &  {\textbf{57.4}}  &  {\textbf{75.5}}  &  {\textbf{76.3}} \\
Big Bird  &  {\transparent{0.3}{2.03}}  &  {\transparent{0.3}{63.9}}  &  {\textbf{71.6}}  &  {\textbf{73.3}}  &  {\textbf{87.1}}  &  {\transparent{0.8}{87.0}}  &  {\transparent{0.3}{1.02}}  &  {\transparent{0.3}{31.9}}  &  {\textbf{57.6}}  &  {\textbf{74.9}}  &  {\textbf{75.4}} \\
H-Transformer-1D  &  {\transparent{0.8}{0.97}}  &  {\textbf{29.3}}  &  {\transparent{0.3}{0.5}}  &  {\transparent{0.3}{6.1}}  &  {\transparent{0.8}{35.4}}  &  {\transparent{0.8}{35.2}}  &  {\transparent{0.8}{0.47}}  &  {\textbf{14.6}}  &  {\transparent{0.3}{43.7}}  &  {\transparent{0.3}{63.6}}  &  {\transparent{0.3}{64.0}} \\
Scatterbrain  &  {\transparent{0.3}{2.23}}  &  {\transparent{0.3}{78.7}}  &  {\transparent{0.8}{60.6}}  &  {\transparent{0.3}{ - }}  &  {\transparent{0.3}{ - }}  &  {\transparent{0.3}{ - }}  &  {\transparent{0.3}{1.04}}  &  {\transparent{0.3}{78.7}}  &  {\transparent{0.3}{18.7}}  &  {\transparent{0.3}{46.6}}  &  {\transparent{0.3}{48.2}} \\
MRA-2  &  {\textbf{0.73}}  &  {\textbf{28.1}}  &  {\textbf{68.9}}  &  {\textbf{73.1}}  &  {\transparent{0.8}{86.8}}  &  {\textbf{87.1}}  &  {\textbf{0.36}}  &  {\textbf{14.0}}  &  {\transparent{0.8}{56.4}}  &  {\transparent{0.8}{73.1}}  &  {\transparent{0.8}{74.1}} \\
MRA-2  &  {\transparent{0.8}{0.86}}  &  {\textbf{34.3}}  &  {\textbf{71.9}}  &  {\textbf{73.8}}  &  {\textbf{87.1}}  &  {\textbf{87.2}}  &  {\transparent{0.8}{0.43}}  &  {\transparent{0.8}{17.1}}  &  {\textbf{57.3}}  &  {\transparent{0.8}{73.7}}  &  {\transparent{0.8}{74.3}} \\
MRA-2-s  &  {\textbf{0.66}}  &  {\textbf{23.8}}  &  {\transparent{0.8}{67.2}}  &  {\transparent{0.8}{72.8}}  &  {\textbf{87.0}}  &  {\textbf{87.0}}  &  {\textbf{0.31}}  &  {\textbf{11.9}}  &  {\transparent{0.8}{56.7}}  &  {\textbf{74.7}}  &  {\textbf{75.1}} \\
MRA-2-s  &  {\textbf{0.80}}  &  {\textbf{29.1}}  &  {\textbf{71.8}}  &  {\textbf{73.8}}  &  {\textbf{87.4}}  &  {\textbf{87.4}}  &  {\textbf{0.38}}  &  {\textbf{14.6}}  &  {\textbf{57.5}}  &  {\textbf{74.2}}  &  {\textbf{75.1}} \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{center}
\vspace{-0.1in}
\caption{Summary of 512 length RoBERTa-base models. We show runtime and memory efficiency, MLM accuracy, and MNLI accuracy. Unit for time (and memory) is ms (and MB). Before and After denote the accuracy before and after finetuning. The m and mm denote the matched and mismatched MNLI. {\color{red} Some methods have more than one row of measurements for different model-specific hyperparameters. We divide measurements into three partitions by ranking and use different fonts for better visualization.} 
}
\label{tab:roberta-base-512}
\vspace{-0.1in}
\end{table*}

==> inserts/sp_pattern_fig_main.tex <==

\begin{figure}[!htbp]
\centering
\includegraphics[width=2.5in]{figs/sparsity_patterns.png}
\caption{\color{red}The top 3 plots are the optimal supports for 3 typical self-attention matrices at $80$\% sparsity. The bottom 3 plots are supports found via our MRA-2 at $80$\% sparsity. }
\label{fig:sp_pattern_main}
\end{figure}

==> inserts/wavelet_transform_qk.tex <==

\begin{figure}[!htbp]
\centering
\includegraphics[width=6in]{figs/wavelet_qkt.png}
\caption{A wavelet analysis and reconstruction applied to a $Q K^T$. The left plot is the true $Q K^T$. The middle plot is the approximation by keeping $10\%$ of wavelet coefficients using Haar basis. A 1D wavelet analysis was performed on each column of $Q$ and each row of $K^T$, and the coefficients of the wavelet decompostions were modified by setting $90\%$ of the smallest coefficients to zero. The altered, and much sparser, wavelet decompositions were used to construct new matrices $\widehat{Q}$ and $\widehat{K}$, and their product $\widehat{Q}\widehat{K}^T$ is shown. The right plot is a similar approximation using ``Daubechies 3''. }
% The wavelet operator used was the  filter. The reconstructed matrix has the same rank as the original, namely 25. ({\em Right}) The absolute difference $|QK'-\widehat{Q}\widehat{K}'|$ between reconstruction and the original is displayed.}
\label{fig:figwavelets}
\end{figure}

==> unused/analysis_unused.tex <==
\subsection{Analysis}

\begin{lemma}
\label{lem:error_bound_of_B}
Assume for all $i \in I, j \in J$, $\mathcal{P}_{i,j} \in [a, a + r]$ for some $a$ and $r > 0$, then 
\begin{equation*}
B_{I,J} \leq B^*_{I,J} \leq \sqrt{C} B_{I,J}
\end{equation*}
where $C = 2 + \exp(2r) - 2 \exp(r)$
\end{lemma}

\begin{proposition}
\label{prop:error_bound_of_attn}
Let $b$ be block size and $\epsilon > 0$, then 
\begin{equation*}
\begin{split}
||D (\mathcal{A}_{BS} - \mathcal{A})||_F &\leq \frac{\epsilon \sqrt{C}}{M} \\
||D (\mathcal{A}_{BS} + \mathcal{A}_{LR} - \mathcal{A})||_F &\leq \frac{\epsilon \sqrt{C - 1}}{M}
\end{split}
\end{equation*}
\end{proposition}
where $M = \inf_i (\frac{1}{n} \sum_{j=1}^n \exp(\mathcal{P}_{i,j}))$

% Assume for all $i \in I, j \in J$ $\mathcal{P}_{i,j} \in [a, a + r]$ for some $a$ and $r > 0$, then by S.SIMIC, Jensen’s inequality and new entropy bounds
% \begin{equation*}
% \begin{split}
% B^*_{I,J} &\leq B_{I,J} + \exp(a) + \exp(a + r) - 2 \exp(a + \frac{r}{2})) \\
% &= B_{I,J} + \exp(a) + \exp(a)\exp(r) - 2 \exp(a) \exp(\frac{r}{2})) \\
% &= B_{I,J} + \exp(a) (1 + \exp(r) - 2 \exp(\frac{r}{2}))
% \end{split}
% \end{equation*}



==> unused/unused.tex <==
\subsection{Block Sparsity}


Then, partition the matrix into $b \times b$ blocks. Consider again the optimization $|| \mathcal{A}_{LR} ||_F + \lambda || \mathcal{A}_{S} ||_0$ constraints on block sparsity

The optimal solution is 
\begin{equation}
(\mathcal{B}^*_{I,J})^2 = \frac{1}{b^2} \sum_{i \in I} \sum_{j \in J} \exp(2 \mathcal{P}_{i, j})
\label{eq:optimal_block_value}
\end{equation}
However, computing this require $O(n^2)$

By the assumption, we can use a lower bound of the above with error bound guarantee on the difference between these two quantities. 
\begin{equation}
(\mathcal{B}_{I,J})^2 = \exp(\frac{2}{b^2} \sum_{i \in I} \sum_{j \in J} \mathcal{P}_{i, j})
\label{eq:block_value}
\end{equation}

\begin{lemma}
\label{lem:error_bound_of_B}
Assume for all $i \in I, j \in J$, $\mathcal{P}_{i,j} \in [a, a + r]$ for some $a$ and $r > 0$, then 
\begin{equation*}
B_{I,J} \leq B^*_{I,J} \leq \sqrt{C} B_{I,J}
\end{equation*}
where $C = 2 + \exp(2r) - 2 \exp(r)$
\end{lemma}

Therefore, we get a solution for $|| \mathcal{A}_{LR} ||_F + \lambda || \mathcal{A}_{S} ||_0$ with guarantee on the difference to the optmial solution. 

\subsection{Finding Low Rank Component}

So far, we have $\mathcal{A}_{LR} = \mathcal{A} - \mathcal{A}_{S} \in mathcal{R}^{n \times n}$, we would need to find a low rank decomposition of $\mathcal{A}_{LR}$

We can use SVD, but it requires $O(n^3)$ complexity

a solution can just set $\mathcal{A}_{LR} = 0$, then the error $|| \mathcal{A}_{LR} + \mathcal{A}_{S} - \mathcal{A} ||$ is 
\begin{proposition}
\label{prop:error_bound_of_attn}
Let $b$ be block size and $\epsilon > 0$, then 
\begin{equation*}
\begin{split}
|| \mathcal{A}_{LR} + \mathcal{A}_{S} - \mathcal{A} || &\leq n \epsilon \sqrt{C} \\
\end{split}
\end{equation*}
\end{proposition}

Alternatively, we find have already computed a low rank approximation of $\mathcal{A}_{LR}$
\begin{equation}
\mathcal{A}_{LR} = \mathcal{U}_{\mathcal{B}} \odot \textbf{1}_{\mathcal{U}_{\mathcal{B}} \leq \epsilon} V
\label{eq:bs_lr_attn}
\end{equation}
Equipped with this low rank component
\begin{proposition}
\label{prop:error_bound_of_attn}
Let $b$ be block size and $\epsilon > 0$, then 
\begin{equation*}
\begin{split}
||\mathcal{A}_{BS} + \mathcal{A}_{LR} - \mathcal{A}||_F &\leq n \epsilon \sqrt{C - 1}
\end{split}
\end{equation*}
\end{proposition}

\input{inserts/bslr_demo_figure}

\subsection{Block Sparsity}

Sparse matrix operations are usually much slower than their theoretical efficiency. Due to the high memory latency and scattered memory access pattern of sparse matrix operations, the memory access latency is a huge bottleneck for sparse matrix operation. It is a well known memory-bound operation. While memory latency hiding and access aligning is optimized for dense matrix operations, this is not an option for sparse matrices. 

Can we do anything about it? We would like to design a sparsity mechanism which has minimal inductive bias on the structures of self-attention matrices and yet efficient enough to compete with dense matrix operation. Consider the inputs to self-attention, Since the nearby tokens are semantically closed, the key and query vectors transformed from nearby tokens are likely to be spatially closed and thus have similar response to the same query and key respectively. As a result, if we divide the self-attention matrix into small blocks, the entries of the same blocks are likely to have similar values. In the other word, nonzero entries of self-attention matrices are usually clustered within blocks. 

Luckily, a type of sparsity, called block sparsity, fits exactly this structure. Block sparsity with optimized execution pipeline is able to align memory access and hide memory latency similar to dense matrices. It is explored in \cite{openai} as an efficient subclass of sparse matrix operations. Further, block sparsity is flexible enough to cover arbitrary sparsity patterns with sufficient nonzero blocks. 

\subsection{Dynamic Sparsity}

Another challenge of efficient sparse approximation is that only the $Q, K, V$ are given and self-attention matrices are unknown and should never be materialized, so we cannot know exactly the location of nonzero entries. Many sparse self-attention methods rely on the predetermined sparsity pattern via prior knowledge. For example, Longformer and Big Bird restricts self-attention to be a local attention. When certain tokens require global attention, an additional global attention component is manually added. Big Bird also add attention to some random tokens, but since self-attention matrices are sparse, uniformly randomly selecting token is less likely to pick tokens with high dependency. 

While in many settings, self-attention matrices are banded matrices and thus local attention is sufficient, it is not always the case. Neither of these two methods can adaptively adjust their sparsity patterns to different self-attention matrices. On the other hand, our goal is to design a mechanism such that sparsity pattern can be efficiently computed and dynamically capture the sparsity of the true self-attention matrices. 

Consider a nonnegative matrix, the optimal sparse approximation in the sense of minimizing Frobenius norm is given by setting the entries with values smaller than certain threshold to zeros. When the block sparsity constraint is imposed, the optimal approximation is similar. Let us partition the $n \times n$ self-attention matrix into $b \times b$ blocks and index the blocks with sets $I, J$ such that $i,j$ entries of a matrix are in block $I, J$ if $i \in I, j \in J$. Define the block values to be normalized Frobenius norm of the blocks 
\begin{equation}
(\mathcal{B}^*_{I,J})^2 = \frac{1}{b^2} \sum_{i \in I} \sum_{j \in J} \exp(2 \mathcal{P}_{i, j})
\label{eq:optimal_block_value}
\end{equation}
The optimal approximation is given by keeping the blocks with $(\mathcal{B}^*_{I,J})^2$ larger than a threshold to be non-zeros and setting the rests to zeros. 

While \eqref{eq:optimal_block_value} is optimal, it cannot be efficiently computed since computing all block values incurs a $O(n^2)$ cost. However, we are not interested in \eqref{eq:optimal_block_value} itself. Rather, we just use it to determine nonzero blocks. We can slightly twist the formulation such that the block values can be efficiently computed and served as a good approximation for \eqref{eq:optimal_block_value}. Consider the alternative block value criterion, 
\begin{equation}
(\mathcal{B}_{I,J})^2 = \exp(\frac{2}{b^2} \sum_{i \in I} \sum_{j \in J} \mathcal{P}_{i, j})
\label{eq:block_value}
\end{equation}
By moving the average into the exponential, we compute a lower bound of \eqref{eq:optimal_block_value}.  \eqref{eq:block_value} can be efficiently computed as follow. Define $\tilde{Q}$ and $\tilde{K}$ such that 
\begin{equation}
\tilde{X}_I = \frac{1}{b} \sum_{i \in I} X_{i}
\label{eq:segmean}
\end{equation}
then $\mathcal{B}_{I,J}$ is simply $\exp(\tilde{Q}_I \tilde{K}_J^T)$. In fact, the $\tilde{Q}$ and $\tilde{K}$ are the segment mean (or local average pooling) used for landmark generation in Nystromformer. Then, our block sparse approximation of self-attention can be written as 
\begin{equation}
\mathcal{A}_{BS} = (\exp( \mathcal{P}) \odot \textbf{1}_{\mathcal{U}_{\mathcal{B}} > \epsilon}) V
\label{eq:bs_attn}
\end{equation}
where $\epsilon > 0$ be the threshold for sparsity and $\mathcal{U}_{\mathcal{B}} \in \R^{n \times n}$ is the up-sampled matrix of $\mathcal{B} \in \R^{n/b \times n/b}$ such that $(\mathcal{U}_{\mathcal{B}})_{i,j} = \mathcal{B}_{I,J}$ for $i \in I, j \in J$. 

\subsection{Low Rank Component}

As the self-attention values computed in nonzero blocks are exactly the same as standard self-attention, the approximation error only come from the zero blocks. 
While the dynamic block sparse approximation perform well by itself, if we can approximate the zero blocks as well, the performance might be further improved. Luckily, we found that a byproduct from $\mathcal{A}_{BS}$ computation, $\mathcal{U}_{\mathcal{B}}$, is a low rank approximation of self-attention matrix. It can be further utilized for approximation of zero blocks without significant overhead. And the resulting block sparsity + low rank approximation can be written as $\mathcal{A}_{BS+LR} = \mathcal{A}_{BS} + \mathcal{A}_{LR}$ where 
\begin{equation}
\mathcal{A}_{LR} = \mathcal{U}_{\mathcal{B}} \odot \textbf{1}_{\mathcal{U}_{\mathcal{B}} \leq \epsilon} V
\label{eq:bs_lr_attn}
\end{equation}
The low rank component $\mathcal{A}_{LR} \in \R^{n \times d}$ can be efficiently computed since it is the up-sampled matrix of $\mathcal{B} \odot \textbf{1}_{\mathcal{B} \leq \epsilon} \tilde{V}  \in \R^{n/b \times d}$ where $\tilde{V}$ is computed according to Eq. \ref{eq:segmean} and $\mathcal{B}$ is reused from block sparsity computation. 

\input{analysis}



% In low rank methods, the complexity is lower bounded by their underlying constraints on self-attention matrix rank. A hyperparameter is introduced for each low rank methods which bounds the rank of self-attention matrix. 

Before get into sparse and low rank decomposition, let us start with a discussion on the limitation of sparsity and low rank. Many of efficient self-attention methods can be divided into two categories: low rank approximation like Linformer, Nystromformer, and Performer and sparse approximation such as Reformer, Longformer, and Big Bird. The efficiency is achieved for longer sequence by restricting the rank or the sparsity of self-attention matrices. To start our discussion, we first evaluate the validity of low rank and sparsity assumption for self-attention matrices. 

The linear complexity of low rank self-attention is achieved by fixing the rank upper bound of self-attention matrices. For example, Nystromformer fixes the number of landmarks, and Performer fixes the random feature dimension when sequence length is increasing. Similarly, sparse approximation achieves linear cost by setting the number of nonzero entries to be linear to sequence length. For example, Longformer and Big Bird fix the window size of local attention. 

\input{inserts/lr_vs_sp_figure}

To evaluate the potential of these two categories of approximations, we set aside the efficiency consideration and assess the validity of low rank and sparsity for self-attention with the best possible approximation methods. Taking $Q, K, V$ from a pretrained RoBERTa model and materializing the standard self-attention matrices, we use truncated SVD of attention matrices for low rank self-attention approximation, and we use the sparse matrices minimizing the distance to the true dense matrices in terms of Frobenius norm for sparse approximation. The results are shown in Fig. \ref{fig:lr_vs_sp}. Ideally the lines should be parallel to the x axis meaning that with fixed target approximation accuracy the rank or average number of non-zeros per row does not increase as sequence length increases, and thus the complexity is linear. 

However, as the figure suggested, the rank of self-attention matrices need to increase almost linear with sequence length to get the same level of approximation accuracy. As a result, when the applications is more demanding on the self-attention mechanism, the limited representation capability of low rank self-attention might result in severe performance degradation. 

On the other hand, the required average number of non-zeros per row only increases slightly as sequence length increases. The sparse approximation seems to have a possibility of much more workload reduction. While sparse approximation gives better trade off between theoretical efficiency and approximation accuracy for self-attention, there are two main challenges for efficient sparse approximation: sparse matrix operation is slow on GPU, and sparsity patterns are unknown without the access to true self-attention matrices. 

Given a self attention matrix, one can 
\begin{equation}
\begin{split}
\min_{\mathcal{A}_{LR}, \mathcal{A}_{S}} & \text{rank}(\mathcal{A}_{LR}) + \lambda || \mathcal{A}_{S} ||_0 \\
\text{s.t. \ \ \ } & || \mathcal{A}_{LR} + \mathcal{A}_{S} - \mathcal{A} || \leq \epsilon
\end{split}
\label{eq:hp_hard_sp_lr_d}
\end{equation}
for $\epsilon \geq 0$

Robust PCA $|| \mathcal{A}_{LR} ||_* + || \mathcal{A}_{S} ||_1$ polynomial time

We have seem that low rank approximation might not be not sufficient for long sequence, while sparsity is limited when the entropy of self-attention is large. Scatterbrain proposed to use low rank + sparse approximation, however, Robust PCA is not efficient. Is it possible to derive a good approximation of low rank + sparsity? 

H-Transformer-1D propose to use H-matrix for self-attention as a generalization for low rank approximation such that off-diagonal is low rank while diagonal is high rank. Via such approximation, interaction among local tokens is precise while dependency to distant tokens is approximated in lower resolution. This can be viewed as low rank approximation on off-diagonal entries plus sparse approximation on diagonal entries. However, this limited the ability of self-attention to capture long range dependency.
